Behavior Uncloning: Distilling Mode Redirection into Policy Weights without Inference-Time Steering

Behavior-cloned policies often learn multiple behavior modes from demonstration datasets, including modes that are unsafe or otherwise undesired at deployment. For example, a policy trained on diverse handover demonstrations may learn to pass a knife blade-first. Standard remedies such as data curation and inference-time steering either require access to the original demonstrations for full retraining or add substantial inference-time overhead. To address this gap, we propose MoRE(Mode Redirection), which redirects policy rollouts toward desired behavior modes through a short "uncloning" step. Specifically, MoRE distills the redirection signal from a temporary mode classifier into the policy weights to steer behavior. A retain loss balances this edit by preserving desired-mode competence, allowing the standalone policy to suppress unwanted modes with zero inference-time overhead. Across eight simulated and real-world tasks, MoRE improves the average deployment success rate (SR) by 44 percentage points over the original mixed-mode policy. Among all compared adaptation and steering baselines, MoRE achieves the strongest SR and approaches the filtered-data retraining reference, while preserving task competence and inference speed. MoRE also generalizes across robot policy backbones, including Diffusion Policy and the Pi0.5 VLA, diverse task categories, and real-world deployments.

==> EXAMPLE/Tables/benchmark_stats.tex <==
\begin{table*}[!htb]
\centering
    \caption{\textbf{Statistics of different training datasets.} We report $<$images available in the dataset$>/<$images used for our training$>$.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrr}
    \toprule
    Dataset             &  Argoverse2                 & Waymo                          & Nuscenes                          &     ScanNet++                      & Taskonomy                          & HM3d                          & Matterport3d \\
    \midrule
    \addlinespace[0.3em]
    Number of images                      &  3.5M/1M    & 1M/700K    & 200K/200K                         & 10M/1M                         & 4M/4M                         & 9M/9M                         & 190K/190K \\
    \bottomrule
\end{tabular}
}
\label{tab:benchmark_stats}
\vspace{-3mm}
\end{table*}

==> EXAMPLE/Tables/hyper_params.tex <==
\begin{table*}[!htb]
\centering
    \caption{\centering \textbf{Hyper-parameters of different experiments.}}
\resizebox{1\textwidth}{!}{
\begin{tabular}{@{}lrrrr}
    \toprule
    Experiment             &  3b SFT                 & 7b SFT                          & 12b SFT                          &     3b GRPO                  \\
    \midrule
    \addlinespace[0.3em]
    Number of training samples            &    35M      &  60M      &  23M                          &       -                   \\
    Learning rate            &   5.2e-5       &  1.0e-4      &  5.6e-5                          &       1.0e-5                   \\
    Learning rate schedule            &     Cosine with linear warmup     &    Cosine with linear warmup    &             Cosine with linear warmup               &    Constant                 \\
    Warmup ratio            &     0.1     &    0.1    &     0.1                       &          -           \\
    Batch size            &     1280     &    1280    &       384                     &             32        \\
    FSDP            &     Yes     &    Yes    &            Yes                &          No           \\
    Gradient clipping            &     0.1     &    0.5    &     1.0                       &         1.0            \\
    Gradient checkpointing            &     Yes     &    Yes    &     Yes                       &           Yes          \\
    Bfloat16  &     Yes     &    Yes    &     Yes                       &           Yes          \\
    Flash Attention 2  &     Yes     &    Yes    &     Yes                       &           Yes          \\
    Unified Focal Length  & 1000 pixels & 1000 pixels & 750 pixels & 1000 pixels \\
    
    
    
    \bottomrule
\end{tabular}
}
\label{tab:hyper-params}
\vspace{-3mm}
\end{table*}

==> EXAMPLE/Tables/main_CV.tex <==
\definecolor{lightgray}{gray}{0.7}

\begin{table*}[t]
\centering
    \caption{\textbf{Comparison with pure vision models.} For pure vision models, we use the numbers reported in~\citep{unidepthv2}, and~\citep{depthpro} if some numbers do not exist in~\citep{unidepthv2}. ``-'' means no result reported in previous papers.
    The last column reports the relative accuracy improvement of pure vision models over our model, i.e., $(\delta_1^\text{CV}-\delta_1^\text{Ours})/\delta_1^\text{Ours}$. Our model is the \emph{first} VLM that has comparable accuracy to pure vision models.}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{}lrrrrrr}
    \toprule
    \multirow{2}{*}{$\delta_1 (\uparrow)$\ \text{of different methods}}            & \multicolumn{2}{c}{\cellcolor{blue!20}\textit{Out}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Out+In}} & \multicolumn{2}{c}{\cellcolor{red!20}\textit{In}} & \\
                                                      & DDAD                          & Nuscenes                          & ETH3D                                                   & sunRGBD                          & ibims1                           & vs Ours ($\uparrow$)\\

    \midrule
    \addlinespace[0.2em]
    \textsc{ZoeDepth}                   & 0.272    & 0.283                         & 0.350                                                & 0.867                         & 0.580                              &    -42.8\%   \\
    \textsc{DepthAnything}                     & -    & 0.354                         & 0.093                                             & 0.850                         & 0.714                                & -40.3\%             \\
    \textsc{DepthAnythingV2}                     & -    & 0.171                         & 0.363                                                 & 0.724                         & -                    & -48.5\%       \\
    \textsc{Metric3D}                     & -    & 0.723                         & 0.456                                            & 0.154                         & 0.797                              & -36.6\%              \\
    \textsc{Unidepth}                     & 0.858                         & 0.846   & 0.185                                              & 0.943                         & 0.157                                     & -27.3\%        \\
    \textsc{Depth Pro}                    & 0.299    & 0.566                         & 0.397                                             & 0.831                         & 0.823                                     & -29.1\%          \\
    \textsc{Metric3Dv2}                    & -    & 0.841                         & 0.900                                                 & 0.812                         & 0.684                         & -3.8\%             \\
    \textsc{UnidepthV2}                     & 0.882    & 0.870                         & 0.852                                                 & 0.964                         & 0.945                                & +9.2\%           \\
    \midrule
        \textsc{Ours (7b)}                           & 0.747    & 0.865                         & 0.718                                                & 0.859                         & 0.920                          & -               \\
    \bottomrule
\end{tabular}
}
\label{tab:main_result_cv}
\vspace{-3mm}
\end{table*}


==> EXAMPLE/Tables/main_result.tex <==
\definecolor{lightgray}{gray}{0.7}

\begin{table*}[t]
\centering
    \caption{\textbf{VLM result.} We tune the prompt for VLMs that are not trained directly on our task to maximize their performance. State-of-the-art VLMs including GPT-5 have only below 0.4 $\delta_1$. \methodname, though orders of magnitudes smaller, achieves an over 2x improvement.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrrrr}
    \toprule
    \multirow{2}{*}{$\delta_1 (\uparrow)$\ \text{of different methods}}            & \multicolumn{3}{c}{\cellcolor{blue!20}\textit{Out}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Out+In}} & \multicolumn{4}{c}{\cellcolor{red!20}\textit{In}} & \\
                            &  Argoverse2                          & DDAD                          & NuScenes                          & ETH3D                          & ScanNet++                          & sunRGBD                          & iBims1                          & NYUv2 & Average \\
    \midrule
    \addlinespace[0.3em]
     \rowcol\multicolumn{10}{c}{\cellcolor{gray!20}\textit{Naive Prediction with Constant Answers}} \\
     \addlinespace[0.2em]
    \textsc{Always Output 2.0m} & 0.006 & 0.010 & 0.010 & 0.106 & 0.305 & 0.384 & 0.280 & 0.383 & 0.186\\
    \addlinespace[0.2em]
    \rowcol\multicolumn{10}{c}{\cellcolor{gray!20}\textit{VLMs}} \\
    \addlinespace[0.2em]
    \textsc{Qwen2.5-VL (3b)}                       & 0.133     & 0.083    & 0.090                         & 0.087                         & 0.120                         & 0.134                         & 0.080                         & 0.128         &   0.106  \\
    \textsc{Qwen2.5-VL (7b)}                       & 0.077     & 0.120    & 0.070                         & 0.126                         & 0.135                         & 0.089                         & 0.160                         & 0.168            &   0.118  \\
    \textsc{Qwen2.5-VL (72b)}                       &  0.119    & 0.140    & 0.186                         &         0.220                 &          0.272                & 0.276                         & 0.212                         &      0.324 &  0.219  \\
    \textsc{Molmo (7b-D)}                       & 0.200     & 0.132    & 0.200                         & 0.126                         & 0.244                         & 0.299                         & 0.200                         & 0.225            & 0.203    \\
    \textsc{Pixtral (12b)}                       &  0.157   &  0.132  &    0.118                    & 0.141                         & 0.318                         & 0.308                         & 0.270                        & 0.145         & 0.199    \\
    \textsc{Gemini-2.5-Pro} & 0.280 & 0.252 & 0.365 & 0.328 & 0.380 & 0.270 & 0.466 & 0.394 & 0.342\\
    \textsc{GPT-o3} & 0.208 & 0.283 & 0.309 & 0.305 & 0.375 & 0.426 & 0.375 & 0.470 & 0.344 \\
    \textsc{GPT-5} & 0.218 & 0.302 & 0.382 & 0.313 & 0.428 & 0.471 & 0.307 & 0.540 & 0.370 \\
     \addlinespace[0.2em]
     \rowcol\multicolumn{10}{c}{\cellcolor{gray!20}\textit{Spatial VLMs}} \\
     \addlinespace[0.2em]
     \textsc{SpaceLLaVA (13B)}                       &  0.100    &  0.067   &   0.083                       &       0.090                   &         0.269                 &                   0.233       &           0.208              &      0.178  & 0.154    \\
     \textsc{SpatialRGPT (8B)}                       &   0.055   &  0.046   &      0.100                    &         0.220                 &             0.346             &                  0.369        &            0.240             &      0.265  & 0.205   \\
    \addlinespace[0.2em]
     \rowcol\multicolumn{10}{c}{\cellcolor{gray!20}\textit{VLMs Trained on Metric Depth Estimation}} \\
     \addlinespace[0.2em]
    \textsc{Seed1.5-VL (official setup)} & 0.009 & 0.012 & 0.013 & 0.219 & 	0.495 & 0.321 & 0.459 & 0.412 & 0.243\\
    \textsc{Seed1.5-VL (our prompt) } & 0.040 & 0.074 & 0.028 & 0.309 & 0.593 & 0.689 & 0.627 & 0.841 & 0.400\\
    \addlinespace[0.2em]
    \midrule
    \textsc{Ours (3b)}                       & 0.808     & 0.724    & \textbf{0.870}                         & \textbf{0.745}                         & 0.838                         & 0.850                         & 0.890                         & 0.868          & 0.824  \\
    \textsc{Ours (7b)}                       & \textbf{0.833}     & \textbf{0.747}    & 0.865                         & 0.718                         & \textbf{0.850}                         & \textbf{0.859}                         & \textbf{0.920}                         & \textbf{0.915}  & \textbf{0.838}               \\
    \textsc{Ours - Pixtral (12b)}                       & 0.734     & 0.670    & 0.819                         & 0.653                         & 0.834                         & 0.786                         & 0.870                         & 0.799     & 0.771           \\
    \bottomrule
\end{tabular}
}
\label{tab:main_result}
\vspace{-3mm}
\end{table*}


==> EXAMPLE/Tables/multiTask.tex <==
\begin{table*}[!htb]
\centering
    \caption{\centering \textbf{MultiTask performance on individual datasets.}}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrrrr}
    \toprule
    \multirow{2}{*}{Method}            & \multicolumn{3}{c}{\cellcolor{blue!20}\textit{Out}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Out+In}} & \multicolumn{4}{c}{\cellcolor{red!20}\textit{In}}\\
                            &  Argo                          & DDAD                          & Nuscenes                          & ETH3D                          & ScanNet++                          & sunRGBD                          & ibims1                          & NYUv2  & Avg $\delta_1 (\uparrow)$ \\
    \midrule
    \addlinespace[0.3em]
    \textsc{Distance}                       & 0.809     & 0.728    & 0.850                         & 0.708                         & 0.856                         & 0.843                         & 0.950                         & 0.876          & 0.828      \\
    \textsc{Principal axis distance}                       & 0.809     & 0.683    & 0.850                         & 0.744                         & 0.846                         & 0.856                         & 0.960                         & 0.896       &    0.831      \\
    \textsc{Speed}                       & 0.801     & 0.722    & 0.843                         & 0.721                         & 0.844                         & 0.819                         & 0.935                         & 0.854         &    0.817    \\
    \textsc{Time}                       & 0.799     & 0.722    & 0.843                         & 0.722                         & 0.842                         & 0.817                         & 0.936                         & 0.846         &    0.816    \\
    \textsc{Two point Distance}                       & 0.651     & 0.423    & 0.670                         & 0.479                         & 0.784                         & 0.727                         & 0.760                         & 0.759         & 0.657       \\
    \textsc{Pose}                       & 0.989     & -    & 0.762                         & -                         & -                         & -                         & -                         & -         &    0.876    \\
    \bottomrule
\end{tabular}
}
\label{tab:multiTask}
\vspace{-3mm}
\end{table*}


==> EXAMPLE/Tables/multiTask_avg.tex <==
\begin{table*}[t]
\centering
    \caption{\textbf{Multi-task result.} Since not all datasets have pose labels, we train the pose task on Argoverse2 and evaluate on Argoverse2 and Nuscenes.}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrrr}
    \toprule
    \multirow{2}{*}{$\delta_1 (\uparrow)$\ \text{on different tasks}}            & \multicolumn{2}{c}{\cellcolor{blue!20}\textit{Single image single point}} & \multicolumn{2}{c}{\cellcolor{green!20}\textit{Reasoning}} & {\cellcolor{red!20}\textit{Multi-point}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Multi-image}}\\
                            &  Distance                                                & Principal axis distance                                                    & Speed                          & Time         & Two point distance                 & Pose & Average \\
    \midrule
    \addlinespace[0.3em]
    \textsc{Always output 2.0}                       & 0.186        & 0.172                                           &                 0.087         &        0.094         & 0.119         & 0.189  & 0.141 \\
    \textsc{Qwen2.5-VL (7B)}                       & 0.118        & 0.085                                         & 0.136                         & 0.087                & 0.066         & 0.048  & 0.09                            \\
    \textsc{SpaceLLaVA (13B)}                       & 0.154        & 0.163                                          & 0.116                         & 0.122                & 0.157         &  0.047  &          0.127                    \\
    \textsc{SpatialRGPT (8B)}                       & 0.205        & 0.132                                         & 0.167                         & 0.122                & 0.143         &  0.195  &          0.161                    \\
    SEED1.5-VL (our prompt) & 0.400 & 0.174 & 0.223 & 0.119 & 0.101 & 0.000 &  0.170\\
    Gemini-2.5-Pro & 0.342 & 0.209  & 0.213 & 0.209 & 0.140 & 0.025 & 0.189 \\
    GPT-5  & 0.370 & 0.241  & 0.199 & 0.181 & 0.150 & 0.120 & 0.210\\
    \textsc{Ours (7B)}                       & \textbf{0.828}       & \textbf{0.831}                                              & \textbf{0.817}                         & \textbf{0.816}            & \textbf{0.657}             & \textbf{0.876}        &  \textbf{0.804}          \\
    \bottomrule
\end{tabular}
}
\label{tab:multiTask_avg}
\vspace{-3mm}
\end{table*}


==> EXAMPLE/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/benchmark_stats.tex <==
\begin{table*}[!htb]
\centering
    \caption{\textbf{Dataset or benchmark statistics.} Replace these placeholders with the data sources, splits, or annotation counts used in your paper.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrr}
    \toprule
    Split & Dataset 1 & Dataset 2 & Dataset 3 & Dataset 4 & Dataset 5 & Dataset 6 & Dataset 7 \\
    \midrule
    \addlinespace[0.3em]
    Training samples & -- & -- & -- & -- & -- & -- & -- \\
    Validation samples & -- & -- & -- & -- & -- & -- & -- \\
    Test samples & -- & -- & -- & -- & -- & -- & -- \\
    Annotation types & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
\end{tabular}
}
\label{tab:benchmark_stats}
\vspace{-3mm}
\end{table*}


==> tables/hyper_params.tex <==
\begin{table*}[!htb]
\centering
    \caption{\centering \textbf{Training hyper-parameters.} Replace these placeholders with the configuration used for each model or experiment.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrr}
    \toprule
    Hyper-parameter & Baseline Setup & Ours -- Small & Ours -- Medium & Ours -- Large \\
    \midrule
    \addlinespace[0.3em]
    Training samples & -- & -- & -- & -- \\
    Learning rate & -- & -- & -- & -- \\
    Learning rate schedule & -- & -- & -- & -- \\
    Batch size & -- & -- & -- & -- \\
    Optimizer & -- & -- & -- & -- \\
    Training steps & -- & -- & -- & -- \\
    Precision & -- & -- & -- & -- \\
    \bottomrule
\end{tabular}
}
\label{tab:hyper-params}
\vspace{-3mm}
\end{table*}


==> tables/main_CV.tex <==
\begin{table*}[t]
\centering
    \caption{\textbf{Comparison with additional baselines.} Use this table for comparisons against another model family, prior system, or external benchmark.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrr}
    \toprule
    Method & Benchmark 1 & Benchmark 2 & Benchmark 3 & Benchmark 4 & Benchmark 5 & Notes \\
    \midrule
    \addlinespace[0.2em]
    \textsc{Baseline 1} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
    \textsc{Baseline 2} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
    \textsc{Baseline 3} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
    \textsc{Baseline 4} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & -- \\
    \midrule
    \textsc{Ours} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & -- \\
    \bottomrule
\end{tabular}
}
\label{tab:main_result_cv}
\vspace{-3mm}
\end{table*}


==> tables/main_result.tex <==
\begin{table*}[t]
\centering
    \caption{\textbf{Main quantitative results.} Replace the metric names, datasets, and values with the main results for your paper.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrrr}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{\cellcolor{blue!20}\textit{Group 1}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Group 2}} & \multicolumn{4}{c}{\cellcolor{red!20}\textit{Group 3}} & \\
                            & Dataset 1 & Dataset 2 & Dataset 3 & Dataset 4 & Dataset 5 & Dataset 6 & Dataset 7 & Dataset 8 & Average \\
    \midrule
    \addlinespace[0.3em]
    \rowcol\multicolumn{10}{c}{\cellcolor{gray!20}\textit{Baselines}} \\
    \addlinespace[0.2em]
    \textsc{Baseline 1} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Baseline 2} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Baseline 3} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \addlinespace[0.2em]
    \midrule
    \textsc{Ours} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} \\
    \bottomrule
\end{tabular}
}
\label{tab:main_result}
\vspace{-3mm}
\end{table*}


==> tables/multiTask.tex <==
\begin{table*}[!htb]
\centering
    \caption{\centering \textbf{Detailed task results.} Use this table when you want to report each task across individual datasets or evaluation subsets.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrrrr}
    \toprule
    \multirow{2}{*}{Task} & \multicolumn{3}{c}{\cellcolor{blue!20}\textit{Group 1}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Group 2}} & \multicolumn{4}{c}{\cellcolor{red!20}\textit{Group 3}}\\
                          & Dataset 1 & Dataset 2 & Dataset 3 & Dataset 4 & Dataset 5 & Dataset 6 & Dataset 7 & Dataset 8 & Average \\
    \midrule
    \addlinespace[0.3em]
    \textsc{Task 1} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Task 2} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Task 3} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Task 4} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \bottomrule
\end{tabular}
}
\label{tab:multiTask}
\vspace{-3mm}
\end{table*}


==> tables/multiTask_avg.tex <==
\begin{table*}[t]
\centering
    \caption{\textbf{Average results across tasks.} Replace the task names and scores with the task-level summary for your paper.}
{\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}lrrrrrrr}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c}{\cellcolor{blue!20}\textit{Task Group 1}} & \multicolumn{2}{c}{\cellcolor{green!20}\textit{Task Group 2}} & \multicolumn{1}{c}{\cellcolor{red!20}\textit{Task Group 3}} & \multicolumn{1}{c}{\cellcolor{yellow!20}\textit{Task Group 4}} & \\
                            & Task 1 & Task 2 & Task 3 & Task 4 & Task 5 & Task 6 & Average \\
    \midrule
    \addlinespace[0.3em]
    \textsc{Baseline 1} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Baseline 2} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \textsc{Baseline 3} & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
    \midrule
    \textsc{Ours} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} & \textbf{0.00} \\
    \bottomrule
\end{tabular}
}
\label{tab:multiTask_avg}
\vspace{-3mm}
\end{table*}

